Commutative Banach Algebras Generated by Toeplitz Operators on the Bergman Space

We present and study commutative Banach algebras generated by Toeplitz operators with generalized quasi-radial pseudo-homogeneous symbols acting on the Bergman space over the unit ball. We develop the Gelfand theory of these algebras and give some structural information about them. In particular, we provide a description of the radical of these algebras. This paper generalizes and completes the results from previous works related to Toeplitz operators with quasi-radial quasi-homogeneous symbols.

==> Pseudo-Applications.tex <==
\section{Examples and applications}

\subsection{Spectral invariance}

\begin{prop}
We will prove that all algebras $\cT_\lambda(\bold{d}_x)$ are
spectral invariant. In particular, for $C\in\cT_\lambda(\bold{d}_x)$,
we have
\[
\spc_{\cT_\lambda(\bold{d}_x)}(C)
=
\spc_{\cL(\cA_\lambda^2(\bB^n))}(C).
\]
\end{prop}
\begin{proof}
Let $A\in\widetilde{\cT_\lambda(\bold{d}_x)}$
of the form
\[
A=\sum_{\rho\in F_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m},
\]
$\psi\in M(\cT_\lambda(\bold{d}_x))$
and, using this data, let $(g_l^{(R)})_l$ as in Theorem
\ref{Maximal ideal space Tdx}.

Let $\cA^*$ be the $C^*$-algebra generated by
$D_{\gamma_\rho}$, $\rho\in F_A$
and $T_{\phi_j^{x_j}}^{\rho_j}$, $j=1,\ldots,m$.
Since the limit in Corollary \ref{Berezin limit Tf-f}
depends only of the nature of the symbol of the operator,
by the same arguments as in the proof of Proposition
\ref{Maximal ideal space Tdx}, we have a well-defined
function
\[
\Psi(C)=\lim_{l\to\infty}\pdi{Cg_l^{(R)},g_l^{(R)}},
\]
for every $C\in\cA^*$ and such that
$\Psi|_{\cT_\lambda(\bold{d}_x)}=\psi$.

Moreover, by Corollary \ref{Berezin limit Tf-f} and relations
\eqref{Tj gl eigenvalues} and \eqref{diagonal gl}
we have
\[
\left|\|Ag_l^{(R)}\|-|\psi(A)|\right|
\leq
\|Ag_l^{(R)}-\psi(A) g_l^{(R)}\|\to0,
\quad l\to\infty.
\]

Thus, if $A$ is invertible, we must have
$A^{-1}\in\cA^*$ and so
\[
1=|\lim_{l\to\infty}\pdi{A^{-1}Ag_l^{(R)},g_l^{(R)}}|
\leq
\|A^{-1}\||\psi(A)|.
\]
So $\psi(A)\neq0$ and, since $\psi$ was arbitrary, this implies
$A^{-1}\in\cT_\lambda(\bold{d}_x)$.

Finally, let $A\in\cT_\lambda(\bold{d}_x)$ be invertible
in $\cL(\cA_\lambda^2(\bB^n))$ and let
$(A_l)_l$ be a sequence in
$\widetilde{\cT_\lambda(\bold{d}_x)}$ that
converges to $A$.
Since the invertible group is open,
we can asume that all elements $(A_l)$ are invertible
in $\cL(\cA_\lambda^2(\bB^n))$.
By our previous reasonings, for every $l=1,2,\ldots$, we have
$A_l^{-1}\in\cT_\lambda(\bold{d}_x))$ for every $l=1,2,\ldots$
and, since inversion is continuous,
$A^{-1}\in\cT_\lambda(\bold{d}_x))$.
\end{proof}

\subsection{The radical $\Rad(\cT_\lambda(\bold{d}_x)))$}

In this section we will assume that all generators $T_{{\phi_j}^{x_j}}$
are different from zero.

\begin{comment}

We recall the notation introduced in Section \ref{Algebra T k-qr}.
Consider the set of indices
\[
\BJ=\{j\in\{1,\ldots,m\}\colon
x_j>0\text{ and }p_{(j)}\neq(0)
\]
and let $\theta_0\in\Theta$ be such that
$J_{\theta_0}=\BJ$.

Following the notation introduced in Section 6 of
\cite{Bauer2015}, for a multi-index
$\bold{1}\neq\theta\in\Theta$
we define the closed ideal $\cI_\infty(\theta)$
in $\cT_\lambda(L_{k-qr}^\infty)$ by
\[
\cI_\infty(\theta)=
\left\{
D_\gamma\in\cT_\lambda(L_{k.qr}^\infty)\colon
\mu(D_\gamma)=0\text{ for all }
\mu\in M_\theta\subset M_\infty
\right\}.
\]

We have $D_\gamma\in\cI_\infty(\infty)$ if and only if
for each $\ka_\theta\in\bZ_+^\theta$
\[
\lim_{m(k_{\cmp{\theta}})\to\infty}
\gamma(\sigma(\ka_\theta,\ka_{\cmp{\theta}}))=0,
\]
where $m(\ka_{\cmp{\theta}})=\min_{j\in J_{\cmp{\theta}}}\ka_j$,
and $\sigma$ is the permutation of $m$-tuples such that
$(\ka_\theta,\ka_{\cmp{\theta}})=
\sigma^{-1}(\ka_1,\ldots,\ka_m)$.

For every
$\ka'\in\bZ_+^{\cmp{\theta}}
=\bigoplus_{j\in\Jt}\bZ_+(j)$,
let $P^{\Jt}_{\ka'}$ be the orthogonal projection
which maps $\cA_\lambda^2(\bB^n)$ onto the subspace
\[
\cj{\spn}
\{
e_\alpha\colon |\alpha_{(j)}|\leq\ka'_j,
\forall~j\in\Jtc
\}.
\]

\begin{lem}
\label{Ideal infty projections density}
The ideal $\cI_\infty(\theta)$ is generated by the projections
$P^{J_\theta}_{\ka'}$, $\ka'\in\bZ_+^{\cmp{\theta}}$.
\end{lem}
\begin{proof}
Clearly we have $P^{\Jt}_{\ka'}\in\cI_\infty(\theta)$.
Conversely, if $D_\gamma\in\cI_\infty(\theta)$,
then $D_\gamma-P_{\ka'}^{\Jt}D_\gamma$ is a diagonal operator with
\[
(D_\gamma-P_{\ka'}^{\Jt}D_\gamma)e_\alpha=
\begin{cases}
\gamma(\alpha)e_\alpha,&\quad
|\alpha_{(j)}|\geq\ka'_j,\enspace\forall~j\in\Jtc,\\
0,&\quad\text{otherwise}.
\end{cases}
\]
This implies that
$\|D_\gamma-P_{\ka'}^{\Jt}D_\gamma\|\to0$,
as $m(\ka')=\min_{j\in\Jtc}\ka'_j\to\infty$.
\end{proof}

Let $\cI(\theta)$ be the closed ideal generated by
$\cI_\infty(\theta)$ and the operators
$T_{\phi_j^{x_j}}$, $j\in\{1,\ldots,m\}$.

\begin{lem}
The inclusion
\[
\cI(\theta)\cap\widetilde{\cT_\lambda(\bold{d}_x)}\subset\cI(\theta)
\]
is norm dense.
\end{lem}
\begin{proof}
Let $T\in\cI(\theta)$ and let $\varepsilon>0$.
There is some $A\in\cT_\lambda(\bold{d}_x)$
such that $\|T-A\|<\varepsilon/2$.
Since $T\in\cI(\theta)$,
by Lemma \ref{Ideal infty projections density},
there is some
$\ka'\in\bZ_+^{\cmp{\theta}}$ such that
$\|P_{\ka'}^{\Jt}T-T\|<\varepsilon/2$.
Therefore
\[
\|T-P_{\ka'}^{\Jt}A\|\leq
\|T-P_{\ka'}^{\Jt}T\|
+
\|P_{\ka'}^{\Jt}T-P_{\ka'}^{\Jt}A\|
<\varepsilon.
\]
\end{proof}

We note that for every $j\in\Jt$ and $M\in\bZ_+$
there is some
$\alpha(j,M)\in\bZ_+^{k_j}$ such that
$|\alpha^j|=N$ and
\[
T_{\phi_j^{x_j}}e_\alpha=0,
\]
for every $\alpha\in\bZ_+^n$ with $\alpha_{(j)}=\alpha^j$.

For each $\alpha\in\bZ^+$,
let $\tau_\alpha$
be the bijection of $\bZ_+^n$ such that interchanges
$\alpha$ and $\tau(\alpha)$, where
\[
\tau(\alpha)_{(j)}=
\begin{cases}
\alpha(j,|\alpha_{(j)}|),&\quad\text{if }j\in\Jtc,\\
\alpha_{(j)},&\quad\text{otherwise},
\end{cases}
\]
We also define the diagonal operator
$S_\alpha$ acting on the basic elements of $\cA_\lambda^2(\bB^n)$
by the rule
\[
S_\alpha(e_\beta)=e_{\tau(\beta)},
\quad \beta\in\bZ_+^n.
\]

Thus, by construction,
for every $\alpha\in\bZ_+^n$ we have
\begin{equation}
\label{P action Txj}
T_{\phi_j^{x_j}}S_\alpha(e_\alpha)=
\begin{cases}
0,&\quad\text{if }j\in\Jtc,\\
T_{\phi_j^{x_j}}S_\alpha(e_\alpha)=
S_\alpha T_{\phi_j^{x_j}}(e_\alpha),&
\quad\text{otherwise}.
\end{cases}    
\end{equation}


Furthermore, since $|\tau_\alpha(\beta)|=|\beta|$ for every
$\beta\in\bZ_+^n$, we also have
\begin{equation}
\label{P action Dg}
D_\gamma S_\alpha(e_\alpha)
=
\gamma(|\alpha|)S_\alpha(e_\alpha)
=S_\alpha\gamma(|\alpha|)(e_\alpha)
=S_\alpha D_\gamma(e_\alpha)
\end{equation}
Thus, for any $A\in\widetilde{\cT_\lambda(\bold{d}_x)}$ of the form
\[
A=\sum_{\rho\in F_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m}
\]
we have
\[
AS_\alpha e_\alpha=
\sum_{\rho\in F'_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m}
e_\alpha,
\]
where
\[
F'_A=\{
\rho\in F_A\colon
\rho_j\neq0,\forall~j\in\Jtc
\}.
\]

Now we define the operator
\[
\cP_{\theta}\colon
\widetilde{\cT_\lambda(\bold{d}_x)}
\cap\cI(\theta)\to
\widetilde{\cT_\lambda(\bold{d}_x)}\cap\cI(\theta)
\]
by extending by linearity the relation
\[
\cP_{\theta}(T)e_\alpha
=
S_\alpha^{-1}TS_\alpha(e_\alpha),\quad\alpha\in\bZ_+^n,
\]
for $T\in\cT_\lambda(\bold{d}_x)$.

\begin{prop}
The operator $\cP_\theta$ is continuous and thus can
be extended to the whole close ideal $\cI(\theta)$.
\end{prop}
\begin{proof}
Let $A\in\widetilde{\cT_\lambda(\bold{d}_x)}\cap\cI(\theta)$
be of the form
\[
A=\sum_{\rho\in F_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m}.
\]
By our previous calculations, we have $\cP_\theta(A)=A'$,
where
\[
A'=\sum_{\rho\in F'_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m}
\]
and
$F'_A=\{
\rho\in F_A\colon
\rho_j\neq0,\forall~j\in\Jtc
\}$.

Let $\ka'\in\bZ_+^{\cmp{\theta}}$.
By taking the a finite direct sum of some of the operators from
Corollary \ref{Operators Sk} with the identity of
the subspace
$\cA_\lambda(\bB^n)\ominus P_{\ka'}^{\Jt}(\cA_\lambda(\bB^n)$,
we can construct a bounded operator
$S$ in $\cA_\lambda^2(\bB^n) P$ such that
\[
S(P_{\ka'}^{\Jt}A')S^{-1}=
\sum_{\rho\in F'_A}
y^\rho
P_{\ka'}^{\Jt}D_{\gamma_\rho}
T_{b_1}^{\rho_{b_1}}\cdots
T_{b_1}^{\rho_{b_{|\theta|}}},
\]
where $y_j=x_j$ if $x_j>0$ and $p_{(j)}\neq(0)$,
and $y_j=1$, otherwise.
Moreover, we have $\|S\|=1$ and $\|S^{-1}\|=s>0$,
for some positive number $s$.

Since the operator $S(P_{\ka'}^{\Jt}A')S^{-1}$ is normal
we have
\begin{align*}
\|S(P_{\ka'}^{\Jt}A')S^{-1}\|&=r(S(P_{\ka'}^{\Jt}A')S^{-1})\\
&=\sup_{(\mu,\zeta)\in M}
\sum_{\rho\in F'_A}
|y^\rho
P_{\ka'}^{\Jt}\gamma_\rho(\mu)
\zeta_{b_1}^{\rho_{b_1}}\cdots
\zeta_{b_1}^{\rho_{b_{|\theta|}}}|\\
&\leq
\sup_{(\mu,\zeta)\in M}
\sum_{\rho\in F'_A}
|y^\rho
\gamma_\rho(\mu)
\zeta_{b_1}^{\rho_{b_1}}\cdots
\zeta_{b_1}^{\rho_{b_{|\theta|}}}|\\
&\leq r(A').
\end{align*}

Therefore
\[
\|P_{\ka'}^{\Jt}A'\|=
\|S^{-1}(SP_{\ka'}^{\Jt}A'S^{-1})S\|\leq
s\|(SP_{\ka'}^{\Jt}S^{-1})\|\leq sr(A').
\]

On the other hand we have
\[
|\psi(A')|=|\psi(A)|\leq
\|A\|,
\]
for every $\psi\in M$, from which it follows that
\[
\|P_{\ka'}^{\Jt}A'\|\leq sr(A')
\leq s\|A\|.
\]
Since $P_{\ka'}^{\Jt}A'$ converges to $A'$ as
$m(\ka')\to\infty$, we conclude that
\[
\|\cP_\theta(A)\|=\|A'\|\leq s\|A\|,
\]
\end{proof}
















\begin{prop}
\label{Projection P}
The operator $\cP_{\BJ}$ is continuous and $\cP_{\BJ}^2=\cP_{\BJ}$.
\end{prop}
\begin{proof}
$\cP_{\BJ}$ is clearly continuous.
Let $A\in\widetilde{\cT_\lambda(\bold{d}_x)}$ of the form
\[
A=\sum_{\rho\in F_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m}
\]
and define
$F'_A=\{\rho\in F_A\colon \rho_j=0,\forall~j\in\BJ\}$.
Then, by \eqref{P action Txj} and \eqref{P action Dg}, we have
\begin{equation}
\label{P action dense}
\cP_{\BJ}(A)=\sum_{\rho\in F'_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m},
\end{equation}
from which it follows that $\cP_{\BJ}^2(A)=\cP_{\BJ}(A)$.
Since $\cP_{\BJ}$ is continuous and $\cT_\lambda(\bold{d}_x)$
is dense in $\cT_\lambda(\bold{d}_x)$,
we conclude that
$\cP_{\BJ}^2=\cP_{\BJ}$.
\end{proof}

\begin{prop}
We have
\[
(I-\cP_{\BJ})(\cI\cap\widetilde{\cT_\lambda(\bold{d}_x)})
=
\Rad(\cT_\lambda(\bold{d}_x)))\cap\widetilde{\cT_\lambda(\bold{d}_x)}
\]
\end{prop}
\begin{proof}
Let $A\in\cI\cap\widetilde{\cT_\lambda(\bold{d}_x)}$.
By Corollary \ref{I convergence M infty}, we have
\[
\psi(A)=0,
\]
for all $\psi=(\mu,\zeta)\in M(\cT_\lambda(\bold{d}_x))$,
with $\mu\in M_{\cmp{\theta_0}}$.

Furthermore, given $\theta\in\Theta$ with
$\theta\neq\cmp{\theta_0}$, there is some index $j\in\BJ$ such that
$\theta_j=1$. Thus, by Propositon \ref{Tjx eigenvalues} and
Theorem \ref{Maximal ideal space Tdx},
we have $\psi(T_{\phi_j^{x_j}})=0$, for each $j\in\BJ$ and
$\psi=(\mu,\zeta)\in M(\cT_\lambda(\bold{d}_x))$,
with $\mu\in M_{\cmp{\theta_0}}$.

Since, by \eqref{P action dense},
every summand of $(I-\cP_{\BJ})(A)$ has at least a factor
$T_{\phi_j^{x_j}}$ for some $j\in\BJ$, we conclude that
\[
\psi((I-\cP_{\BJ})A)=0,
\]
for each $\psi=(\mu,\zeta)\in M(\cT_\lambda(\bold{d}_x))$,
with $\mu\in M_{\theta}$ and $\theta\neq\theta_0$.

Conversely,
let
$A\in\Rad(\cT_\lambda(\bold{d}_x)))
\cap\widetilde{\cT_\lambda(\bold{d}_x)}$
of the form
\[
A=\sum_{\rho\in F_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m}
\]
and let
$F'_A$ as in the proof of Lemma \ref{Projection P}.
Reasoning as before, we have
\[
\psi(A)=
\sum_{\rho\in F'_A}
\gamma_\rho(\psi)
\]





Then we have $\psi(A)=0$ for every $\psi\in M_{\cmp{\theta_0}}$.
\end{proof}


Let $\ka'\in\bZ_+^{\cmp{\theta}}$.
By taking the a finite direct sum of some of the operators from
Corollary \ref{Operators Sk} with the identity of
the subspace
$\cA_\lambda(\bB^n)\ominus P_{\ka'}^{\Jt}(\cA_\lambda(\bB^n)$,
we can construct a bounded operator
$S$ in $\cA_\lambda^2(\bB^n) P$ such that
\[
S(P_{\ka'}^{\Jt}A')S^{-1}=
\sum_{\rho\in F'_A}
y^\rho
P_{\ka'}^{\Jt}D_{\gamma_\rho}
T_{b_1}^{\rho_{b_1}}\cdots
T_{b_1}^{\rho_{b_{|\theta|}}},
\]
where $y_j=x_j$ if $x_j>0$ and $p_{(j)}\neq(0)$,
and $y_j=1$, otherwise.
Moreover, we have $\|S\|=1$ and $\|S^{-1}\|=s>0$,
for some positive number $s$.

\end{comment}

















































































\begin{prop}
The algebra
$\cT_\lambda(\bold{d}_x)$ is semi-simple
if and only if
either $x_j>0$ or $p_{(j)}=(0)$
for each $j=1,\ldots,m$.
\end{prop}
\begin{proof}
Suppose that $x_j>0$ or $p_{(j)}=(0)$
for each $j=1,\ldots,m$.
Let $T\in\Rad(\cT_\lambda(\bold{d}_x)))$ such that
$T\neq0$. Then there is $\ka\in\bZ_+^m$
such that
$T|_{H_\ka}\neq0$.

By Lemma \ref{Hamel basis}, there is
a Hamel basis of unit vectors
$\{g_\beta\}_{\beta\in I}$ for $H_\ka$ such
that
\[
T_{\phi_1^{x_1}}^{\rho_1}\cdots T_{\phi_m^{x_m}}^{\rho_m}
g_\beta=
\zeta_1^{\rho_1}\cdots\zeta_m^{\rho_m},
\]
for every $\rho\in\bZ_+^m$ and $\beta\in I$.
Thus there is some $\beta_0$ with $Te_{\beta_0}\neq0$.

Nevertheless, for every
$A\in\widetilde{\cT_\lambda(\bold{d}_x)}$
of the form
\[
A=\sum_{\rho\in F_A}D_{\gamma_\rho}
T_{\phi_1^{x_1}}^{\rho_1}\cdots
T_{\phi_m^{x_m}}^{\rho_m},
\]
we have
\[
Ag_{\beta_0}=\sum_{\rho\in F_A}
\gamma_\rho(\ka)
\zeta^\rho=\psi(A)
g_{\beta_0},
\]
where $\psi=(\kappa,\zeta)\in M(\cT_\lambda(\bold{d}_x))$.
Since $\widetilde{\cT_\lambda(\bold{d}_x)}$
is dense in $\cT_\lambda(\bold{d}_x)$, we must have
\[
Ag_{\beta_0}=\psi(A)g_{\beta_0},\quad\forall~A\in
\cT_\lambda(\bold{d}_x).
\]
But then
\[
0\neq T g_{\beta_0}=\psi(T)g_{\beta_0}=0.
\]

Conversely, let $j'$ be such that $x_{j'}=0$
and $p_{(j')}\neq(0)$.
Then, by a similar argument as in
Lemma 6.7 from \cite{Bauer2015},
$D_\gamma T_{\phi_{j'}^{x_{j'}}}$
is topologically nilpotent
for $\gamma\in c_0$. That is,
$D_\gamma T_{\phi_{j'}^{x_{j'}}}
\in\Rad(\cT_\lambda(\bold{d}_x)))$.
\end{proof}




